Class Interference Regularization

Contrastive losses yield state-of-the-art performance for person re-identification, face verification and few shot learning. They have recently outperformed the cross-entropy loss on classification at the ImageNet scale and outperformed all self-supervision prior results by a large margin (SimCLR). Simple and effective regularization techniques such as label smoothing and self-distillation do not apply anymore, because they act on multinomial label distributions, adopted in cross-entropy losses, and not on tuple comparative terms, which characterize the contrastive losses. Here we propose a novel, simple and effective regularization technique, the Class Interference Regularization (CIR), which applies to cross-entropy losses but is especially effective on contrastive losses. CIR perturbs the output features by randomly moving them towards the average embeddings of the negative classes. To the best of our knowledge, CIR is the first regularization technique to act on the output features. In experimental evaluation, the combination of CIR and a plain Siamese-net with triplet loss yields best few-shot learning performance on the challenging tieredImageNet. CIR also improves the state-of-the-art technique in person re-identification on the Market-1501 dataset, based on triplet loss, and the state-of-the-art technique in person search on the CUHK-SYSU dataset, based on a cross-entropy loss. Finally, on the task of classification CIR performs on par with the popular label smoothing, as demonstrated for CIFAR-10 and -100.

==> cuhk-sysu-qualitative_results.tex <==
\tabcolsep 1.0pt
\renewcommand{\arraystretch}{0.5}

\newlength{\cuhkfigheightqrpn}
\setlength{\cuhkfigheightqrpn}{3cm}

\begin{figure*}[h]
\begin{center}
\begin{tabular}{c|cc}
&&&&&&\\
\includegraphics[trim=7cm 2cm 10cm 5cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/12_s14166_gt_11.jpg}
&
\includegraphics[trim=6cm 2cm 9.8cm 5cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/12_s14166_qsse_top0.jpg}
&
\includegraphics[trim=5.5cm 2cm 8cm 3cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/12_s14166_qsse_top1.jpg} 
\\



\includegraphics[trim=11cm 2cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/16_s17426_gt_5.jpg}
&
\includegraphics[trim=0cm 1cm 7.5cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu//16_s17426_qsse_top0.jpg}
&
\includegraphics[trim=0cm 0cm 7cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/16_s17426_qsse_top1.jpg} 
\\

\includegraphics[trim=8cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/14_s17154_gt_2.jpg}
&
\includegraphics[trim=6cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/14_s17154_qsse_top0.jpg}
&
\includegraphics[trim=0cm 0cm 7cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/14_s17154_qsse_top2.jpg} 
\\



\includegraphics[trim=14cm 5cm 1cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/20_s17789_gt_4.jpg}
&
\includegraphics[trim=0cm 0cm 6cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/20_s17789_qsse_top0.jpg}
&
\includegraphics[trim=3cm 0cm 4cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/20_s17789_qsse_top1.jpg} 
\\

\includegraphics[trim=16cm 3cm 0cm 3cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/55_s13147_gt_2.jpg}
&
\includegraphics[trim=13cm 2cm 0cm 3cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/55_s13147_qsse_top0.jpg}
&
\includegraphics[trim=11cm 3cm 4cm 3cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/cuhk-sysu/55_s13147_qsse_top1.jpg} 
\\

Query& \multicolumn{2}{c}{Top-2 Results}\\

\end{tabular}

\end{center}
\caption{Qualitative person search results on the \textbf{CUHK-SYSU} dataset.  In each row, we show the query image in the first column with the bounding box of the queried person in yellow. The second and third columns give the \emph{Top-2} matches retrieved by our method. Correct person match is marked in green bounding box, while a wrong match is marked in red. Note that in person search the inputs are full images unlike cropped bounding boxes in person re-id.}
\label{fig:cuhk-qualitative}
\end{figure*}









==> market1501-qualitative_results.tex <==
\tabcolsep 1.0pt
\renewcommand{\arraystretch}{0.5}

\newlength{\cuhkfigheightqrpn}
\setlength{\cuhkfigheightqrpn}{3cm}

\begin{figure*}[h]
\begin{center}
\begin{tabular}{c|ccccc}
&&&&&&\\
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0004_c2s3_059152_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top001_name_0004_c1s6_016996_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top002_name_0004_c6s3_089517_01.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0004_c1s6_017046_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top004_name_0004_c1s6_027096_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top005_name_0004_c6s3_089492_01.jpg}

&\\



\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0009_c6s1_000476_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top001_name_0009_c1s1_000451_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top002_name_0009_c1s1_000401_02.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0009_c5s1_000476_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top004_name_0087_c4s1_013951_02_redbox.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top005_name_0009_c5s1_000551_02.jpg}

&\\



\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0018_c5s1_001776_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top001_name_0018_c4s1_002351_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top002_name_0018_c1s1_001851_01.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0018_c2s1_001226_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top004_name_0018_c1s1_001926_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top005_name_0018_c3s1_001526_01.jpg}

&\\

\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0041_c1s6_015171_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top001_name_0041_c6s3_087667_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top002_name_0041_c2s3_057652_02.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0041_c2s3_057627_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top004_name_0041_c5s3_076062_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top005_name_0041_c3s3_063969_01.jpg}

&\\

\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0050_c2s1_004801_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top001_name_0050_c3s1_004976_02.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top002_name_0050_c3s1_004926_02.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0050_c6s1_005551_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top004_name_0479_c2s1_124991_02_red.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top005_name_0165_c2s1_029676_03_red.jpg}


&\\
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, cfbox=yellow 2pt 2pt, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0050_c2s1_004801_00.jpg}
&
\frame{\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0041_c1s6_015171_00.jpg}}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn, cfbox=green 2pt 2pt]{Pictures/result_images/market-1501/gallery_top001_name_0050_c3s1_004976_02.jpg} 
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0009_c6s1_000476_00.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/gallery_top003_name_0009_c5s1_000476_01.jpg}
&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheightqrpn]{Pictures/result_images/market-1501/query_top000_name_0004_c2s3_059152_00.jpg}


&\\


Query& \multicolumn{5}{c}{Top-5 Results}\\

\end{tabular}


\end{center}
\caption{Qualitative Results on the \textbf{Market-1501} person re-identification dataset. The first column shows the query image. The next columns give the \emph{Top-5} results retrieved by our proposed method. Results marked in red are false positives.}
\label{fig:market1501-qualitative}
\end{figure*}









==> no_cite_mini_tiered_sota_sorted.tex <==
\begin{table*}
\small
\begin{center}
\begin{tabular}{lcccc}

& \multicolumn{2}{c}{\textit{miniImageNet}} & \multicolumn{2}{c}{\textit{tieredImageNet}}\\
\hline
Method & \textbf{1-shot}  & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot}  \\
\hline
\hline

Matching Net [64], NIPS16 &  43.6 &  55.3 & - & - \\

Meta-learner LSTM [51], ICLR17 & 43.4 &  60.6  & - & - \\
MAML [9], ICML17  & 48.7   &  63.1& -  &  -\\
Meta-SGD [34], arXiv 2017 & 54.2  & 70.9 & - & - \\
ProtoNet [58], NIPS17 & 49.4  & 68.2 & 53.3 & 72.7\\

ProtoNet [68] (ResNet18), ICLR18 &  54.1 &  73.7 & -& -\\



Large Margin (Triplet) [67], NIPS18 & 50.1 &  66.9& - & -\\
REPTILE [45], arXiv18 & 49.9 & 65.9  & - & -\\


Relation Net [60], CVPR18 & 50.4 &  65.3& 54.5 & 71.3 \\
Dynamic [15], CVPR18 &  56.2 & 73.0 & - & - \\
Predict Params [48], CVPR18 & 59.6  & 73.7 & - & -  \\
SNAIL [40], ICLR18 & 55.7  & 68.9 & -  & - \\

TADAM [46], NIPS18  & 58.5 & 76.7 & - &- \\

Soft k-means [52], ICLR18 & - & - &52.4 &  69.9 \\
Transductive Prop [36], ICLR19 & 55.5 & 69.9& 59.9  & 73.3 \\
Projective Subspace [57], arXiv19 &  - & 68.1 & - & 71.2 \\
Incremental [53], NIPS19 & 54.9  & 63.0  & 56.1 &65.5\\
IDeMe-Net [6], CVPR19   & 57.7 & 74.3 & - & -\\
Individual [17], ICLR19 & 56.9 & 70.5 & -& - \\
CAML [25], ICLR19 & 59.2 & 72.3  & - & - \\
LEO [55], ICLR19 & 61.8  & 77.6  & \textbf{66.3} & 81.4\\

MetaOptNet [31], CVPR19 & \textbf{62.6}  & \textbf{78.6} & 65.9 & \textbf{81.5}\\
Global Class Rep. [32], ICCV19 &  53.2 & 72.3 & - & -\\





\hline
Triplet&  57.4 & 70.2 & 63.9 & 77.1 \\
 + \textit{CIR} & \textbf{58.4} & \textbf{72.6} & \textbf{64.3} & \textbf{77.7}\\
 
\hline
Cross Entropy $\rightarrow$ Triplet & 57.7 & 74.3 & 66.6 & 81.7\\
 + \textit{CIR} & \textbf{60.5} & \textbf{75.8} & \textbf{69.1} & \textbf{82.9} \\
\hline


\end{tabular}
\end{center}
\caption{
\small CIR on few shot learning for 5-way 1-shot and 5-way 5-shot. The average accuracy of 600 randomly generated episodes is reported for miniImageNet [64] and tieredImageNet [52].
}
\label{tab:mini_tiered}
\end{table*}




==> psearchteaser.tex <==
\begin{figure}[h]
\centering
\includegraphics[trim=0cm 8.8cm 0cm 1.3cm, clip=true, width=0.8\linewidth]{./Pictures/Psearch_teaser.pdf}
\caption{\small Illustration of Class Interference Regularization (CIR) for the task of person search. The Table of Average Class embeddings (TAC) is shared with the OIM table of re-identification network. Based on the TAC, we randomly perturb each person id feature embedding according to the average embedding of wrong id.}
\label{fig:Psearch}
\end{figure}

==> qualitative.tex <==
\section{Qualitative Results}\label{sec:qualitativesupp}
In this section, we illustrate sample results of person re-identification, person search and few-shot learning obtained by regularizing the given baselines with CIR.

Figure~\ref{fig:market1501-qualitative} and~\ref{fig:cuhk-qualitative} show some results for person re-identification and person search respectively. Note that person re-identification uses cropped images of people whereas person search uses full images with bounding box annotations. Our proposed CIR is applicable to both of them. Finally, in Figure~\ref{fig:tieredImagenet-qualitative}, we show some results for few-shot classification. For each task, the experimental setup, dataset and evaluation metric are as described in Section \ref{sec:exp} of the main paper.

\input{Pictures/market1501-qualitative_results}

\input{Pictures/cuhk-sysu-qualitative_results}

\input{Pictures/tieredImagenet-qualitative_results}

==> tieredImagenet-qualitative_results.tex <==
\tabcolsep 1.0pt
\renewcommand{\arraystretch}{0.5}


\begin{figure*}[h]
\begin{center}
\begin{tabular}{cccccc}

&&&&&&\\


\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_1_query_1_name_n0787515200000836.jpg}
&
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_1_support_0_0_name_n0289460500000368.jpg} 
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=blue 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_1_support_1_0_name_n0787515200000917.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_1_support_2_0_name_n0928863500000481.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_1_support_3_0_name_n0432654700000629.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_1_support_4_0_name_n0404930300000015.jpg}


\\

\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_14_query_3_name_n0216545600000617.jpg}

&

\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_14_support_0_0_name_n0769753700000488.jpg} 
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true ]{Pictures/result_images/tiered-Imagenet/Episode_14_support_2_0_name_n0282342800000076.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_14_support_3_0_name_n0216545600000408.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=red 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_14_support_1_0_name_n0771847200000729.jpg}
&



\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_14_support_4_0_name_n0774958200000072.jpg}
\\







\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_5_query_2_name_n0787380700000463.jpg} 
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_5_support_0_0_name_n0264024200000782.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_5_support_1_0_name_n0306359900000120.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=blue 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_5_support_2_0_name_n0787380700000617.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_5_support_3_0_name_n0149633100000162.jpg}
&
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_5_support_4_0_name_n0393031300000945.jpg}


\\

\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_4_query_0_name_n0282342800000967.jpg} 
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=blue 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_4_support_0_0_name_n0282342800001134.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_4_support_1_0_name_n0775359200001274.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_4_support_2_0_name_n0210904700000260.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_4_support_3_0_name_n0149633100001112.jpg}
&
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_4_support_4_0_name_n0758411000001121.jpg}

\\
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_3_query_1_name_n0227625800001077.jpg} 
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_3_support_0_0_name_n0363309100000449.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=green 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_3_support_1_0_name_n0227625800000543.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_3_support_2_0_name_n0946860400000955.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_3_support_3_0_name_n0223604400000109.jpg}
&
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_3_support_4_0_name_n0260605200000100.jpg}




\\

\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_10_query_3_name_n0772087500000269.jpg}
&
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_10_support_0_0_name_n0771741000000880.jpg} 
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_10_support_1_0_name_n0211018500000118.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_10_support_2_0_name_n0210842200000436.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_10_support_3_0_name_n0772087500000765.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=red 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_10_support_4_0_name_n0761450000000328.jpg}
\\
\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_6_query_3_name_n0771847200000917.jpg}

&

\includegraphics[scale=0.23, trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_6_support_0_0_name_n0220685600001164.jpg} 
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_6_support_1_0_name_n0216869900000298.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_6_support_2_0_name_n0775311300000230.jpg}
&

\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true, cfbox=blue 2pt 2pt]{Pictures/result_images/tiered-Imagenet/Episode_6_support_3_0_name_n0771847200001234.jpg}
&
\includegraphics[scale=0.23,trim=0cm 0cm 0cm 0cm, clip=true]{Pictures/result_images/tiered-Imagenet/Episode_6_support_4_0_name_n0228178700001026.jpg}

\\
&&&&&&\\
Query & \multicolumn{5}{c}{ 1 (-shot) support example from each of 5 (-way) classes} \\


\end{tabular}
\end{center}

\caption{Qualitative results on \textbf{tieredImageNet} for 5-way 1-shot classification. The first column shows the query image to be classified. The next five columns show 1 (-shot) support example from each of the 5 (-way) classes. For each query image, the support example with highest similarity score is marked. Correctly assigned class is marked with a blue bounding box, while red bounding box represents wrong classification.}

\label{fig:tieredImagenet-qualitative}
\end{figure*}








